Data-Driven Performance Guarantees for Classical and Learned Optimizers

We introduce a data-driven approach to analyze the performance of continuous optimization algorithms using generalization guarantees from statistical learning theory. We study classical and learned optimizers to solve families of parametric optimization problems. We build generalization guarantees for classical optimizers, using a sample convergence bound, and for learned optimizers, using the Probably Approximately Correct (PAC)-Bayes framework. To train learned optimizers, we use a gradient-based algorithm to directly minimize the PAC-Bayes upper bound. Numerical experiments in signal processing, control, and meta-learning showcase the ability of our framework to provide strong generalization guarantees for both classical and learned optimizers given a fixed budget of iterations. For classical optimizers, our bounds are much tighter than those that worst-case guarantees provide. For learned optimizers, our bounds outperform the empirical outcomes observed in their non-learned counterparts.

==> cover/jmlr_coverletter.tex <==
% !TeX root = jmlr_coverletter.tex
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Data-Driven Performance Guarantees for Classical and Learned Optimizers}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript introduces a \red{data-driven approach to analyze the performance of continuous algorithms for parametric optimization} which is important because many \red{worst-case analyses for classical optimizers can be too pessimistic} and \red{learned optimizers lack strong generalization guarantees}.
We use statistical learning theory, namely a sample convergence bound and PAC-Bayes theory, to provide guarantees for both classical and learned optimizers.
We apply our methods to numerous examples in control, signal processing, and meta-learning.
For classical optimizers, our bounds are much tighter than
those that worst-case guarantees provide. 
For learned optimizers, our bounds outperform the empirical outcomes observed in their non-learned counterparts.

% Our architecture consists of a neural network mapping problem parameters to warm starts, followed by a predefined number of fixed-point iterations.
% In this way, the neural network predicts warm-starts with the end-to-end goal of minimizing the downstream loss.
% We apply our methods to numerous examples in control, statistics, and signal processing, observing significantly reduced solution times.



We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{Silvia Villa}, University of Genova (villa@dima.unige.it)
    \item \red{Quentin Berthet}, Google DeepMind (qberthet@google.com)
    \item \red{Stefanie Jegelka}, Massachusetts Institute of Technology (stefje@csail.mit.edu)
    \item \red{Jean-Philippe Vert}, Owkin (jean-philippe.vert@m4x.org)
    \item \red{Shiqian Ma}, Rice University (sqma@rice.edu)
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{Joe Marino}, Google DeepMind (josephmarino@google.com)
    \item \red{Atlas Wang}, University of Texas, Austin (atlaswang@utexas.edu)
    \item \red{Ernest Ryu}, Seoul National University (ernestryu@snu.ac.kr)
    \item \red{Yisong Yue}, California Institute of Technology (yyue@caltech.edu)
    \item \red{Pontus Giselsson}, Lund University (pontusg@control.lth.se)
\end{itemize}

Our submission has the following keywords: \red{learning to optimize}, \red{statistical learning theory}, \red{generalization bounds}, \red{fixed-point iterations}, \red{parametric optimization}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

Rajiv Sambharya (Princeton University)\\
Bartolomeo Stellato (Princeton University)

\end{document}







































